Adapting Speaker Embeddings for Speaker Diarisation

The goal of this paper is to adapt speaker embeddings for solving the problem of speaker diarisation. The quality of speaker embeddings is paramount to the performance of speaker diarisation systems. Despite this, prior works in the field have directly used embeddings designed only to be effective on the speaker verification task. In this paper, we propose three techniques that can be used to better adapt the speaker embeddings for diarisation: dimensionality reduction, attention-based embedding aggregation, and non-speech clustering. A wide range of experiments is performed on various challenging datasets. The results demonstrate that all three techniques contribute positively to the performance of the diarisation system achieving an average relative improvement of 25.07% in terms of diarisation error rate over the baseline.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> tables/ahc_dihard_ablation.tex <==
\begin{table}[t!]
  \centering
  \begin{tabularx}{\linewidth}{lYYYYY}
  \toprule
  Configuration  & DER & FA & Miss & Conf\\
  \midrule
  \multicolumn{5} {c} {\bf DIHARD 1 Evaluation set} \\
  \midrule
  baseline   & 40.24 & 16.17 & 10.60 & 13.45\\
  + dr    & 40.76 & 16.17 & 10.60 & 13.97\\%p0.9, r0.4609
  + aa    & 39.46 & 16.17 & 10.60 & 12.68\\%p0.9, r0.4609
  + ns    & 37.49 & 14.22 & 10.55 & 12.71\\%p0.9, r0.4609
  + dr + aa    & 38.64 & 16.17 & 10.60 & 11.86\\%p0.9, r0.4609
  + dr + ns    & 35.16 & 14.42 & 10.47 & 10.26\\%p0.9, r0.4609
  + aa + ns    & 37.36 & 14.32 & 10.62 & 12.42\\%p0.9, r0.4609
  + dr + aa + ns   & 33.44 & 13.82 & 11.34 & 8.28\\%p0.9, r0.4609
  \midrule
  Challenge Top-1   & 35.51 & - & - & -\\%p0.9, r0.4609
  \midrule
  \multicolumn{5} {c} {\bf DIHARD 2 Evaluation set} \\ 
  \midrule
    baseline   & 44.15 & 19.17 & 11.67 & 13.31\\
  + dr    & 44.61 & 19.17 & 11.67 & 13.76\\%p0.9, r0.4609
  + aa    & 43.98 & 19.17 & 11.67 & 13.14\\%p0.9, r0.4609
  + ns    & 40.47 & 15.25 & 11.96 & 13.25\\%p0.9, r0.4609
  + dr + aa    & 42.47 & 19.17 & 11.67 & 11.62\\%p0.9, r0.4609
  + dr + ns    & 37.92 & 15.23 & 12.10 & 10.58\\%p0.9, r0.4609
  + aa + ns    & 40.18 & 15.30 & 12.21 & 12.66\\%p0.9, r0.4609
  + dr + aa + ns   & 35.78 & 14.55 & 13.18 & 8.04\\%p0.9, r0.4609
  \midrule
  Challenge Top-1   & 35.10 & - & - & -\\%p0.9, r0.4609
  
%   w/ OSD    & 13.93 & 0.62 & 9.00 & 4.31\\%p0.9, r0.4609
%   w/ OSD    & 14.03 & 0.82 & 8.70 & 4.51\\%p0.8, r0.4609
  
%  None               & a & b & c & d \\ 
%  Segment            & 2.24     & 2.20    & 2.14    \\ 
%  Add label           & 2.09    & 1.62    & 1.17    \\ 
%  Segment\&Add label  & \textbf{2.06}     & \textbf{1.52}    & \textbf{1.09}    \\
  \bottomrule
  \end{tabularx}
%   \caption{Speaker diarization performance using OSD model. `Segment' refers to applying further segmentation on the EPD segment using OSD and `Add label' refers to allocating second best speaker for OSD segments (FA: false alarm, Conf: confusion).}
  \caption{Results on the DIHARD challenge dataset using the baseline with every combination of proposed techniques. (FA: false alarm, Conf: confusion).}
  \label{tab:ahc_dihard1_abl}
\end{table}

==> tables/dihard1_ablation.tex <==
\begin{table}[t!]
  \centering
  \begin{tabularx}{\linewidth}{lYYYYY}
  \toprule
  Configuration  & DER & FA & Miss & Conf\\
  \midrule
  \multicolumn{5} {c} {\bf DIHARD 1 Evaluation set} \\
  \midrule
  baseline   & 49.20 & 16.17 & 10.60 & 22.41\\
  + dr    & 48.74 & 16.17 & 10.60 & 21.96\\%p0.9, r0.4609
  + aa    & 37.01 & 16.17 & 10.60 & 10.22\\%p0.9, r0.4609
  + ns    & 46.15 & 14.55 & 10.26 & 21.33\\%p0.9, r0.4609
  + dr + aa    & 37.43 & 16.17 & 10.60 & 10.65\\%p0.9, r0.4609
  + dr + ns    & 39.67 & 14.52 & 10.37 & 14.77\\%p0.9, r0.4609
  + aa + ns    & 32.83 & 14.11 & 10.60 & 8.10\\%p0.9, r0.4609
  + dr + aa + ns   & 32.93 & 13.99 & 11.23 & 7.70\\%p0.9, r0.4609
  \midrule
  Challenge Top-1   & 35.51 & - & - & -\\%p0.9, r0.4609
  \midrule
  \multicolumn{5} {c} {\bf DIHARD 2 Evaluation set} \\ 
  \midrule
    baseline   & 51.33 & 19.17 & 11.67 & 20.49\\
  + dr    & 51.17 & 19.17 & 11.67 & 20.33\\%p0.9, r0.4609
  + aa    & 41.10 & 19.17 & 11.67 & 10.26\\%p0.9, r0.4609
  + ns    & 47.15 & 16.02 & 11.76 & 19.36\\%p0.9, r0.4609
  + dr + aa    & 41.19 & 19.17 & 11.67 & 10.35\\%p0.9, r0.4609
  + dr + ns    & 41.50 & 15.88 & 12.00 & 13.61\\%p0.9, r0.4609
  + aa + ns    & 35.78 & 14.98 & 12.32 & 8.47\\%p0.9, r0.4609
  + dr + aa + ns   & 35.29 & 14.67 & 13.14 & 7.47\\%p0.9, r0.4609
  \midrule
  Baseline & 50.12 & - & - & -\\%p0.9, r0.4609
  Challenge Top-1   & 35.10 & - & - & -\\%p0.9, r0.4609
  
%   w/ OSD    & 13.93 & 0.62 & 9.00 & 4.31\\%p0.9, r0.4609
%   w/ OSD    & 14.03 & 0.82 & 8.70 & 4.51\\%p0.8, r0.4609
  
%  None               & a & b & c & d \\ 
%  Segment            & 2.24     & 2.20    & 2.14    \\ 
%  Add label           & 2.09    & 1.62    & 1.17    \\ 
%  Segment\&Add label  & \textbf{2.06}     & \textbf{1.52}    & \textbf{1.09}    \\
  \bottomrule
  \end{tabularx}
%   \caption{Speaker diarization performance using OSD model. `Segment' refers to applying further segmentation on the EPD segment using OSD and `Add label' refers to allocating second best speaker for OSD segments (FA: false alarm, Conf: confusion).}
  \caption{Results on the DIHARD challenge dataset using the baseline with every combination of proposed techniques. (FA: false alarm, Conf: confusion).}
  \label{tab:dihard1_abl}
\end{table}

==> tables/dihard1_ablation_ahc_spec.tex <==
\begin{table}[t!]
  \centering
  \caption{Results on the DIHARD I challenge dataset using the baseline with every combination of proposed techniques. (FA: false alarm, MS: missed speech, SC: speaker confusion).}
    \resizebox{\linewidth}{!}{\begin{tabular}{lccccc}
    \Xhline{3\arrayrulewidth}
    %\vspace{4pt}
    Configuration  & DER & FA & MS & SC\\
    \midrule
    \multicolumn{5} {c} {\bf Baseline with spectral clustering} \\
    \midrule
    Baseline   & 49.20 & 16.17 & 10.60 & 22.41\\
    + DR    & 48.74 & 16.17 & 10.60 & 21.96\\%p0.9, r0.4609
    + AA    & 37.01 & 16.17 & 10.60 & 10.22\\%p0.9, r0.4609
    + NS    & 46.15 & 14.55 & 10.26 & 21.33\\%p0.9, r0.4609
    + DR + AA    & 37.43 & 16.17 & 10.60 & 10.65\\%p0.9, r0.4609
    + DR + NS    & 39.67 & 14.52 & 10.37 & 14.77\\%p0.9, r0.4609
    + AA + NS    & 32.83 & 14.11 & 10.60 & 8.10\\%p0.9, r0.4609
    + DR + AA + NS   & 32.93 & 13.99 & 11.23 & 7.70\\%p0.9, r0.4609
    + DR + AA + NS + Oracle SAD  & 16.83 & 0.0 & 8.71 & 8.12\\%p0.9, r0.4609
    \midrule
    \multicolumn{5} {c} {\bf Baseline with AHC} \\ 
    \midrule
    Baseline   & 40.24 & 16.17 & 10.60 & 13.45\\
    + DR    & 40.76 & 16.17 & 10.60 & 13.97\\%p0.9, r0.4609
    + AA    & 39.46 & 16.17 & 10.60 & 12.68\\%p0.9, r0.4609
    + NS    & 37.49 & 14.22 & 10.55 & 12.71\\%p0.9, r0.4609
    + DR + AA    & 38.64 & 16.17 & 10.60 & 11.86\\%p0.9, r0.4609
    + DR + NS    & 35.16 & 14.42 & 10.47 & 10.26\\%p0.9, r0.4609
    + AA + NS    & 37.36 & 14.32 & 10.62 & 12.42\\%p0.9, r0.4609
    + DR + AA + NS   & 33.44 & 13.82 & 11.34 & 8.28\\%p0.9, r0.4609
    + DR + AA + NS + Oracle SAD  & 17.81 & 0.0 & 8.71 & 9.10\\%p0.9, r0.4609
    \midrule
    Track 1 Winner \cite{sell2018diarization}   & 23.73 & - & - & -\\%p0.9, r0.4609
    Track 2 Winner \cite{landini2019but}   & 35.51 & - & - & -\\%p0.9, r0.4609
    
%     w/ OSD    & 13.93 & 0.62 & 9.00 & 4.31\\%p0.9, r0.4609
%     w/ OSD    & 14.03 & 0.82 & 8.70 & 4.51\\%p0.8, r0.4609
    
%    None               & a & b & c & d \\ 
%    Segment            & 2.24     & 2.20    & 2.14    \\ 
%    Add label           & 2.09    & 1.62    & 1.17    \\ 
%    Segment\&Add label  & \textbf{2.06}     & \textbf{1.52}    & \textbf{1.09}    \\
    \Xhline{3\arrayrulewidth}
  \end{tabular}}
%   \caption{Speaker diarization performance using OSD model. `Segment' refers to applying further segmentation on the EPD segment using OSD and `Add label' refers to allocating second best speaker for OSD segments (FA: false alarm, Conf: confusion).}
  \label{tab:dihard1_abl}
\end{table}

==> tables/dihard2_ablation_ahc_spec.tex <==
\begin{savenotes}
  \begin{table}[t!]
    \caption{Results on the DIHARD II challenge dataset using the baseline with every combination of proposed techniques. (FA: false alarm, MS: missed speech SC: speaker confusion).}
    \centering
    % \begin{tabularx}{\linewidth}{lYYYYY}
    % \resizebox{\columnwidth}{!}{\begin{tabular}{|l|l|l|l|l|}

    \resizebox{\linewidth}{!}{\begin{tabular}{lccccc}
      \Xhline{3\arrayrulewidth}
      \vspace{4pt}
      Configuration  & DER & FA & MS & SC\\
      \midrule
      \multicolumn{5} {c} {\bf Baseline with spectral clustering} \\
      \midrule
         Baseline   & 51.33 & 19.17 & 11.67 & 20.49\\
      + DR    & 51.17 & 19.17 & 11.67 & 20.33\\%p0.9, r0.4609
      + AA    & 41.10 & 19.17 & 11.67 & 10.26\\%p0.9, r0.4609
      + NS    & 47.15 & 16.02 & 11.76 & 19.36\\%p0.9, r0.4609
      + DR + AA    & 41.19 & 19.17 & 11.67 & 10.35\\%p0.9, r0.4609
      + DR + NS    & 41.50 & 15.88 & 12.00 & 13.61\\%p0.9, r0.4609
      + AA + NS    & 35.78 & 14.98 & 12.32 & 8.47\\%p0.9, r0.4609
      + DR + AA + NS   & 35.29 & 14.67 & 13.14 & 7.47\\%p0.9, r0.4609
      + DR + AA + NS + Oracle SAD  & 17.98 & 0.0 & 9.68 & 8.29\\%p0.9, r0.4609
      \midrule
      \multicolumn{5} {c} {\bf Baseline with AHC} \\ 
      \midrule
        Baseline   & 44.15 & 19.17 & 11.67 & 13.31\\
      + DR    & 44.61 & 19.17 & 11.67 & 13.76\\%p0.9, r0.4609
      + AA    & 43.98 & 19.17 & 11.67 & 13.14\\%p0.9, r0.4609
      + NS    & 40.47 & 15.25 & 11.96 & 13.25\\%p0.9, r0.4609
      + DR + AA    & 42.47 & 19.17 & 11.67 & 11.62\\%p0.9, r0.4609
      + DR + NS    & 37.92 & 15.23 & 12.10 & 10.58\\%p0.9, r0.4609
      + AA + NS    & 40.18 & 15.30 & 12.21 & 12.66\\%p0.9, r0.4609
      + DR + AA + NS   & 35.78 & 14.55 & 13.18 & 8.04\\%p0.9, r0.4609
      + DR + AA + NS + Oracle SAD  & 18.67 & 0.0 & 9.68 & 8.99\\%p0.9, r0.4609
      \midrule
       Track 1 Winner\footnote{http://dihard.ldc.upenn.edu/competitions/73\#results}    & 18.42 & - & - & -\\%p0.9, r0.4609
  %    Track 2 baseline \cite{ryant2019second}& 50.12 & - & - & -\\%p0.9, r0.4609
       Track 2 Winner\footnote{http://dihard.ldc.upenn.edu/competitions/74\#results}    & 27.11 & - & - & -\\%p0.9, r0.4609
      
  %     w/ OSD    & 13.93 & 0.62 & 9.00 & 4.31\\%p0.9, r0.4609
  %     w/ OSD    & 14.03 & 0.82 & 8.70 & 4.51\\%p0.8, r0.4609
      
  %    None               & a & b & c & d \\ 
  %    Segment            & 2.24     & 2.20    & 2.14    \\ 
  %    Add label           & 2.09    & 1.62    & 1.17    \\ 
  %    Segment\&Add label  & \textbf{2.06}     & \textbf{1.52}    & \textbf{1.09}    \\
      \Xhline{3\arrayrulewidth}
    %   \end{tabularx}
      \end{tabular}}
  %   \caption{Speaker diarization performance using OSD model. `Segment' refers to applying further segmentation on the EPD segment using OSD and `Add label' refers to allocating second best speaker for OSD segments (FA: false alarm, Conf: confusion).}
    \label{tab:dihard2_abl}
  \end{table}
\end{savenotes}

